MVDiffusion: Enabling Holistic Multi-view Image Generation with Correspondence-Aware Diffusion

This paper introduces MVDiffusion, a simple yet effective method for generating consistent multi-view images from text prompts given pixel-to-pixel correspondences (e.g., perspective crops from a panorama or multi-view images given depth maps and poses). Unlike prior methods that rely on iterative image warping and inpainting, MVDiffusion simultaneously generates all images with a global awareness, effectively addressing the prevalent error accumulation issue. At its core, MVDiffusion processes perspective images in parallel with a pre-trained text-to-image diffusion model, while integrating novel correspondence-aware attention layers to facilitate cross-view interactions. For panorama generation, while only trained with 10k panoramas, MVDiffusion is able to generate high-resolution photorealistic images for arbitrary texts or extrapolate one perspective image to a 360-degree view. For multi-view depth-to-image generation, MVDiffusion demonstrates state-of-the-art performance for texturing a scene mesh.

==> texts/4.1-mv-ldm.tex <==
\subsection{Multi-view Latent Diffusion Models}
\label{subsec:mv-ldm}

As demonstrated by Figure~\ref{fig:overview}, our multi-view Latent Diffusion Models extend the original LDMs of Stable Diffusion (SD) in two aspects: 1) the latents of multi-view images are denoised simultaneously (i.e., in parallel) with the shared UNet, and 2) novel correspondence-aware attention (CAA) blocks are inserted into the UNet to learn cross-view geometry consistency and enable global awareness. 

We design two model variants for MVDiffusion to accommodate different types of input conditions: the \textit{text-conditioned generation model} takes text prompts as the condition, while the \textit{image\&text-conditioned generation model} takes the text prompts as well as one or two additional source images. Below, we briefly describe the role of the two models in the context of the concrete generation task:
\begin{itemize}[leftmargin=*,topsep=0pt,itemsep=0pt,noitemsep]
\item \textit{Panorama generation:} Only one of the two models will be used depending on the type of user input. If only texts are given, the text-conditioned model generates eight perspective views in parallel. If an additional source view is presented, the text\&image conditioned model can outpaint seven perspective views considering both the image and text conditions.

\item \textit{Multi-view depth-to-image generation:} Since the input of this task is usually a long sequence of depth maps with known camera poses, generating all images together is usually computationally infeasible. As a workaround,
the text-conditioned generation model first sub-samples a sparse set of depth maps as the ``key frames'' and generates the textured images. Then, the image\&text conditioned model works like an interpolation model, which takes two consecutive key-frame images as the additional condition and generates the images in between. These generated images should be consistent with both the depth maps and two condition images, while also aligning with the text prompts. The image\&text conditioned model runs over all pairs of consecutive key-frame images to densify the generation results.
\end{itemize}

We then describe how these two model variants work in the generation process. 
We start with the text-conditioned model, as the image\&text condition model can be regarded as its extension.

\mypara{Text-conditioned generation model} 
 This model generates multiple images from text prompts and allows users to specify \textit{different prompts for different perspective views}, enhancing the control over the generated content.
Figure~\ref{fig:overview}(Left) illustrates the generation process. The latents of multiple images are initialized with independent Gaussian noises.
At each denoising step, the noisy latents are fed into the multi-branch UNet to perform denoising for all the multi-view latents concurrently, guided by a sampler (\eg, DDIM~\cite{song2020ddim}). After the denoising process finishes in $T$ steps,   the final multi-view latents are decoded by SD's pre-trained VAE decoder into images. The image resolution is $512\times 512$ for the panorama case and $192\times 256$ for the multi-view depth-to-image case. 

The SD UNet consists of several downsample and upsample blocks, while each block is accompanied by a CAA block to enforce multi-view consistency. 
As shown by Figure~\ref{fig:overview} (Right), we initialize the final linear layer of the CAA block to be zeros as suggested in ControlNet~\cite{zhang2023controlnet}, which ensures that our modifications do not disrupt the original functionality of the SD model. 

\mypara{Image\&text-conditioned generation model}
Compared to the text-conditioned generation model, this model generates multi-view target images conditioned on one or two additional source images, while the correspondences between the target and condition images are known. The model works in slightly different ways for the two tasks, and the details are described as follows:

\vspace{-0.3em}\raisebox{0.25ex}{}
\textit{(1) Panoramic image generation:} The goal of the image\&text-conditioned model here is to generate full 360-degree panoramic views (seven target images) based on a single perspective image (one condition image) and the per-view text prompts.
We use SD's impainting model~\cite{stableimpaint} as the base model as it takes one condition image. Similar to the text-conditioned generation model, CAA blocks with zero initializations are inserted into the UNet and trained on our datasets. 

\vspace{-0.3em} 
For the generation process, the model reinitializes the latents of both the target and condition images with noises from standard Gaussians. In the UNet branch of the condition image, we concatenate a mask of ones to the image (4 channels in total). This concatenated image then serves as the input to the inpainting model, which ensures that the content of the condition image remains the same. On the contrary, in the UNet branch for a target image, we concatenate a black image (pixel values of zero) with a mask of zeros to serve as the input, thus requiring the inpainting model to generate a completely new image based on the text condition and the correspondences with the condition image.


\vspace{-0.3em}\raisebox{0.25ex}{} 
\textit{(2) Multi-view depth-to-image generation:} 
As described earlier, the goal of the image\&text-conditioned model in this task is to densify the key-frame images generated by the text-conditioned model, and the additional condition here is a pair of key-frame images.
Since the SD's impainting model does not support depth-conditioning, we have to adopt a different approach here.
Inspired by VideoLDM~\cite{blattmann2023align}, we reuse the depth-conditioned UNet with CAA blocks from the text-conditioned generation model, which has been trained for generating sparse key-frame images given the depth maps and camera poses. Extra convolution layers are inserted to inject the information of two condition images.

\vspace{-0.3em}
We then elaborate on how the additional convolution layers work. Note that these layers are added to each block of the UNet with varying feature map sizes. For the UNet branch of a condition image (there are two condition images), the condition image itself is concatenated with a mask of ones (4 channels), and then a zero convolution operation is used to downsample the concatnated image to the corresponding feature map size. These downsampled conditions are then added to the input of the UNet blocks. For the branch of a target image, we concatenate a black image, whose pixel values are all zero, to a mask of zeros, and apply the same zero convolution operation to downsample the image to match the corresponding feature map size. These downsampled conditions are also added to the input of the UNet blocks. This procedure essentially trains the model such that when the mask is one, the branch regenerates the condition images, and when the mask is zero, the branch generates the in-between target images. At the start of the generation process, the latents of both the target and condition images are initialized with noises from standard Gaussians. 


==> texts/4.2-caa.tex <==
\subsection{Correspondence-aware Attention}
\label{subsec:caa}
\begin{wrapfigure}[12]{r}{7cm}
\vspace{-0.52cm}
\hspace{-0.2cm}
\includegraphics[width=7cm]{texts/figures/attention_multi.pdf}
\caption{Correspondence-aware attention}
\label{fig:correpondence_attn}
\end{wrapfigure}
We now introduce the ``correspondence-aware attention'' (CAA) mechanism, which is the key of MVDiffusion to enforce correspondence constraints across multi-view feature maps (See Figure~\ref{fig:correpondence_attn}). This mechanism operates by taking into account the source feature maps $\feat$ and $N$ target feature maps $\feat^l$ ($l\in [0,N-1]$).
%$\mathbf{C}$.
For a token located at position ($\mathbf{s}$) in the source feature map, we compute the attention output (message) based on the corresponding pixels  $\{\mathbf{t}^l\}$ in the target feature maps $\{\feat^l\}$ (not necessarily at integer coordinates) with local neighborhoods.

Concretely, for each target pixel $\mathbf{t}^l$, we consider a $K\times K$ neighborhood $\mathcal{N}(\mathbf{t}^l)$
by adding integer displacements $(d_x/d_y)$ to the (x/y) coordinate, where $|d_x|< K/2$ and $|d_y|< K/2$. In practice, we use $K=3$ with a neighborhood of 9 points for panorama for quality and $K=1$ for geometry-conditioned multi-view image generation for efficiency.
%offsetting the image coordinate by integers. In practice $k=3$, and we add or subtract 1 from the x or y coordinate to generate the neighborhood.
The message $\mathbf{m}$ is calculated as
\begin{align}
\mathbf{m} &= \sum_l \sum_{t^{l}_{*} \in \mathcal{N}(\mathbf{t}^l)} 
\mbox{SoftMax}\left(
\left[ 
\mathbf{W_Q} \bar{\feat}(\mathbf{s})  \right] \cdot \left[ \mathbf{W_K} \bar{\feat}^l(t^{l}_{*}) \right] \right) \mathbf{W_V} \bar{\feat}^l(t^{l}_{*}), \\
%\bar{\feat} (s) &= \feat(s) + \pe(0), \quad \bar{\feat}(t^{l}_{*}) = \feat^l(t^{l}_{*}) + \pe(s^{l}_{*} - s), \\
\bar{\feat} (\mathbf{s}) &= \feat(\mathbf{s}) + \pe(0), \quad \bar{\feat}^l(t^{l}_{*}) = \feat^l(t^{l}_{*}) + \pe(\mathbf{s}^{l}_{*} - \mathbf{s}).
\end{align}
%

%
The message calculation follows the standard attention mechanism that aggregates information from the target feature pixels $\{t^{l}_{*}\}$ to the source ($s$). $\mathbf{W_Q}$, $\mathbf{W_K}$, and $\mathbf{W_V}$ are the learnable weights of query, key and value matrices. The target feature $\feat^l(t^{l}_{*})$ is not at an integer location and is obtained by bilinear interpolation. The key difference is the added position encoding $\gamma(\cdot)$ to the target feature $\feat^l(t^{l}_{*})$ based on the 2D displacement (panorama) or 1D depth error (geometry) between its corresponding location $\mathbf{s}^{l}_{*}$ in the source image and $\mathbf{s}$. In panorama generation, the displacement provides the relative location in the local neighborhood. In the depth-to-image generation case, the disparity provides cues about depth discontinuities or occlusions, crucial for high-fidelity image generation. Note that a displacement is a 2D (displacement) or 1D (depth error) vector, and we apply a standard frequency encoding~\cite{vaswani2017transformer} to the displacement in both x and y coordinates. 



==> texts/4.3-train.tex <==
\subsection{Training}
\label{subsec:train}

To train MVDiffusion models, we extend the loss of LDMs (Eq.~\ref{eq:cond_ldm_loss}) from single-view to multi-view.
For each training step, we uniformly sample a shared noise level $t$ from $1$ to $T$ for all the multi-view images $\left\{\img_i\right\}_{i=1}^N$, and then employ the following loss function: 
\begin{align}
L_{\tiny{\mbox{MVDiffusion}}}
:= \expec_{\left\{\latent^i = \encoder(\img^i) \right\}_{i=1}^N, \left\{\bepsilon^i \sim \mathcal{N}(0, 1)\right\}_{i=1}^N, \cond, t} \Big[ \sum_{i=1}^N \Vert \bepsilon^i - \model^i(\left\{ \latent_t^i \right\},t, \conditioner(\cond)) \Vert_{2}^{2}\Big].
\label{eq:cond_ldm_loss_ours}
\end{align}
We use $\model^i$ to denote the estimated noise for the $i$-th image. $\latent_t^i$ is the noisy latent for the $i$-th image. Since our training dataset is much smaller than the pre-training dataset of SD models, we freeze the original SD parameters in our training as much as possible to retain the original generalization capability. 
For the panorama generation task, we only train the inserted CAA blocks. 

However, due to the significant resolution difference in the multi-view depth-to-image generation task ($192\times 256$ compared to the $512\times 512$ of the original SD), the SD model has to be fine-tuned, and 
we adopt a two-stage training process. In the first stage, we fine-tune the SD UNet model using all ScanNet data to adjust the resolution. This stage is single-view training (Eq.~\ref{eq:cond_ldm_loss}) without the CAA blocks. In the second stage, we integrate the CAA blocks and the image condition blocks into the UNet, and only these added parameters are trained.


==> texts/table/ablation.tex <==
\begin{table}[]
\centering
\begin{tabular}{ll|ll}
                                                &          & PSNR & PSNR ratio \\ \hline
                                                & GT       & 37.7 & 1.00       \\
\multicolumn{1}{c}{\multirow{2}{*}{Base model}} & W.O CPA  & 10.6 & 0.28       \\
\multicolumn{1}{c}{}                            & With CPA & 25.6 & 0.68       \\
\multirow{2}{*}{SR}                       & W.O. CPA & 28.3 & 0.75       \\
                                                & With CPA & 31.0 & 0.82      
\end{tabular}
\caption{Ablation study on geometry consistency.}
\end{table}


==> texts/table/depth_results_old.tex <==
\begin{wraptable}[8]{r}{7cm}
\centering
\vspace{-1.5em}
\begin{tabular}{llll}
Method   & FID $\downarrow$ & IS $\uparrow$ & CS $\uparrow$ \\ \midrule
RePaint~\cite{lugmayr2022repaint} &  85.91 & 7.15   & 30.21     \\
ControlNet~\cite{zhang2023controlnet} &  55.85 & 7.23   & \textbf{30.31}     \\
Ours     & \textbf{23.10} & \textbf{7.27}   &  \textbf{29.03}         
\end{tabular}
\vspace{-0.5em}
\caption{Comparison in Fréchet Inception Distance (FID), Inception Score (IS), and CLIP Score (CS) for multiview depth-to-image generation.}\label{tab:depths}
\end{wraptable}

==> texts/table/geometry_consistent_old.tex <==

\begin{table}[t]
\begin{minipage}{0.55\textwidth}  % adjust width as needed
\centering
% \small
\vspace{-0.6em}
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l}{Task $\rightarrow$} & \multicolumn{2}{c}{Panorama} & \multicolumn{2}{c}{Depth-to-image} \\
\cmidrule(r){2-3} \cmidrule(r){4-5}
Method                  & PSNR $\uparrow$        & Ratio $\uparrow$       & PSNR $\uparrow$        & Ratio $\uparrow$       \\ 
\midrule
G.T.                                     & 37.7        & 1.00               & 21.41        &  1.00                 \\
SD (Persp.)                       & 10.6        & 0.28                 &  11.2            &  0.44                 \\
Ours                                   &\textbf{31.0}        &  \textbf{0.82}                 & \textbf{17.41}        &   \textbf{0.76}               
\end{tabular}
\caption{Multi-view consistency for panorama generation and multi-view depth-to-image generation.}\label{tab:geo_consistency}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}  % adjust width as needed
\centering
% \small
\vspace{-0.6em}
\begin{tabular}{lccc}
\toprule
  Method  &   CA       & PSNR$\uparrow$ & Ratio$\uparrow$ \\
  \midrule
    \multicolumn{1}{l}{GT} & -    & 37.7 & 1.00       \\ \hdashline
\multicolumn{1}{l}{\multirow{2}{*}{GM}} & \xmark  & 10.6 & 0.28       \\
\multicolumn{1}{c}{}                            & \cmark & 25.6 & 0.68       \\ \hdashline
\multicolumn{1}{l}{\multirow{2}{*}{Ours}}                       & \xmark & 28.3 & 0.75       \\
    & \cmark & \textbf{31.0} & \textbf{0.82}      
\end{tabular}
\caption{Ablation study on multiview consistency with Generation Module (GM) only or full system.}\label{tab:ablation}
\end{minipage}
\end{table}
